VEGETA: Vertically-Integrated Extensions for Sparse/Dense GEMM Tile Acceleration on CPUs

Deep Learning (DL) acceleration support in CPUs has recently gained a lot of traction, with several companies (Arm, Intel, IBM) announcing products with specialized matrix engines accessible via GEMM instructions. CPUs are pervasive and need to handle diverse requirements across DL workloads running in edge/HPC/cloud platforms. Therefore, as DL workloads embrace sparsity to reduce the computations and memory size of models, it is also imperative for CPUs to add support for sparsity to avoid under-utilization of the dense matrix engine and inefficient usage of the caches and registers. This work presents VEGETA, a set of ISA and microarchitecture extensions over dense matrix engines to support flexible structured sparsity for CPUs, enabling programmable support for diverse DL models with varying degrees of sparsity. Compared to the state-of-the-art (SOTA) dense matrix engine in CPUs, a VEGETA engine provides 1.09x, 2.20x, 3.74x, and 3.28x speed-ups when running 4:4 (dense), 2:4, 1:4, and unstructured (95%) sparse DNN layers.

==> sections/04_SW_Backup.tex <==
\subsection{SW Optimizations for GEMM Kernel}
\label{sec:compiler}

%\TODO{Should this be in the Evaluation section?}
% not sure this is needed
\begin{comment}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/tilespmm-example.pdf}
    \caption{Active tiles for algorithm 1.  \AB{Maybe you can add colour to tile register file also. Also sreg numbering renaming}}
    \label{fig:tilespmm-example}
\end{figure}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/matrix_code-2.pdf}
    \caption{Active tiles for algorithm 1. }
    \label{fig:tilespmm-example}
\end{figure}
\end{comment}

%\cjh{This needs an introduction.  We need to explain why we're talking about a GEMM kernel, and only a GEMM kernel.  Perhaps that high level discussion should go even earlier, but it needs to be somewhere.  I suggest saying something along the lines of }

We focus our software discussion on constructing a high-performance GEMM kernel on VEGETA. 
We implemented the software optimizations manually on our kernel, but this could be employed by higher-level DNN libraries/frameworks~\cite{onednn} and/or tensor compilers~\cite{tvm}. 
Moreover, these instructions may also be used by other kernels that rely on matrix multiplication. 
%, including convolution~\cite{convolution}.
%Inspired by Intel's AMX intrinsics for tile computations, 
We have added intrinsics for each of the VEGETA instructions. These VEGETA intrinsics give the programmer or library writer low-level control of inline assembly while retaining readability and ease of programming. Our software infrastructure additionally provides code generation support for these new instructions which a compiler or library developer can use to write and optimize their own kernels.

As an example, \autoref{lst:spmm_base} shows a basic implementation of the GEMM kernel. $T_m, T_n, T_k$ represent the register tile size for each dimension while $D_m, D_n, D_k$ represent the GEMM dimensions. In \autoref{lst:spmm_opt}, we optimize the kernel performance using the following loop transformation techniques to reduce the number of load instructions.

\begin{itemize}
    \item \textbf{Register promotion:} The load from $C[i][j]$ is independent of the innermost loop index, $k$ and therefore there are redundant loads from the same address within the $k$-loop. We store the value of $C[i][j]$ in a register for the duration of the $k$-loop, thereby reducing the total number of loads from $3\times D_m\times D_n\times D_k$ to $2\times D_m\times D_n\times D_k + D_m \times D_n$.
    
    \item \textbf{Loop unroll and jam:} We unroll the outer $i$ loop by a factor of $3$ and fuse the inner loops. This allows for the reuse of $B[j][k]$ across iterations of the $i$-loop, further reducing the number of tile loads to $\frac{4}{3}\times D_m\times D_n\times D_k + D_m\times D_n$. Unrolling also provides the out-of-order scheduler with a larger window of independent instructions, thereby reducing pipeline stalls.
\end{itemize}

Depending on the target CPU's specific memory organization and the performance bottlenecks of the kernel, a user could explore additional transformations to improve cache locality including loop tiling, permutation, kernel fusion and data prefetch~\cite{libxsmm_ipdps20, onednn}, but we leave them as future work for HPC/ML compiler/library developers.
%%%%%%%
\input{algorithms/gemm} \label{gemm-amx}


==> sections/99_authors.tex <==
%%%%%%%%%%%%% comment out for double blind review %%%%%%%%%%%%%%%%%
\begin{comment}
\author{\IEEEauthorblockN{Geonhwa Jeong}
\IEEEauthorblockA{\textit{Georgia Institute of Technology} \\
email address}
\and
\IEEEauthorblockN{Sana Damani}
\IEEEauthorblockA{\textit{Georgia Institute of Technology} \\
email address}
\and
\IEEEauthorblockN{Abhimanyu Bambhaniya}
\IEEEauthorblockA{\textit{Georgia Institute of Technology} \\
email address}
\and
\IEEEauthorblockN{Eric Qin}
\IEEEauthorblockA{\textit{Georgia Institute of Technology} \\
email address}
\and
\IEEEauthorblockN{Christopher J. Hughes}
\IEEEauthorblockA{\textit{Intel Labs} \\
email address}
\and
\IEEEauthorblockN{Sreenivas Subramoney}
\IEEEauthorblockA{\textit{Intel Labs} \\
email address}
\and
\IEEEauthorblockN{Hyesoon Kim}
\IEEEauthorblockA{\textit{Georgia Institute of Technology} \\
email address}
\and
\IEEEauthorblockN{Tushar Krishna}
\IEEEauthorblockA{\textit{Georgia Institute of Technology} \\
email address}
}
\end{comment}







==> tables/registers.tex <==
%\HK{Any significance meaning of names for T,U,V, M tile registers? Or are they just different size tile registers? is "Size" column per register or total?  } 
%\GJ{I started from treg for normal (1kb) tile register. u and v are the next alphabets after t, and I chose those for different sizes. inspired from xmm/ymm/zmm..}

\begin{table}[t] 
\scriptsize
\centering
\caption{VEGETA registers}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Tile Register} 
%& \textbf{Intrinsics} 
& \textbf{Size per Register} 
& \textbf{Number of Registers} \\
%\cline{2-4} 
\hline
\hline

vreg 
%& \_\_tile\_dpbf16ps 
& 4KB
&
\begin{tabular}[c]{@{}c@{}}
2
\end{tabular}
\\
\hline

ureg 
%& \_\_tile\_dpbf16ps 
& 2KB
&
\begin{tabular}[c]{@{}c@{}}
4
\end{tabular}
\\
\hline

treg 
%& \_\_tile\_dpbf16ps 
& 1KB
&
\begin{tabular}[c]{@{}c@{}}
8
\end{tabular}
\\
\hline

mreg 
& 128B
&
\begin{tabular}[c]{@{}c@{}}
8
\end{tabular}
\\
\hline

\end{tabular}
\label{tab1}
\label{table:registers}
\end{table}

==> tables/row-wise-sparsity-evalution.tex <==
\begin{table}[t]
\scriptsize
\centering
\caption{Speedup of Row-wise Sparse DNN layers in VEGETA-S.}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Layer Dimension/Sparsity} & \textbf{RASA} & \textbf{S2TA} & \textbf{Vegeta} \\
\hline
\hline
M=3136,	N=64, K=256/60 & 100 & 100  & 60\\
\hline
M=3136,	N=64, K=256/70 & 100 & 100 & 20 \\
\hline
M=3136,	N=64, K=256/80 & 100 & 100 & 20 \\
\hline
M=3136,	N=64, K=256/90 & 100 & 100 & 20 \\
\hline
M=3136,	N=64, K=256/95 & 100 & 100 & 20 \\
\hline
M=3136,	N=64, K=256/98 & 100 & 100 & 20 \\
\hline
\end{tabular}
\label{table:row-wise-speedup}
\end{table}

==> tables/systolic-array-option.tex <==
\begin{table}[t] 
\scriptsize
\centering
\caption{Trade-offs for different RF and SA}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Configurations} 
%& \textbf{Intrinsics} 
&
\begin{tabular}[c]{@{}c@{}}
\textbf{Efficient}\\
\textbf{Register Usage}
\end{tabular}
&
\begin{tabular}[c]{@{}c@{}}
\textbf{Efficient}\\
\textbf{Array Usage}
\end{tabular}
& \textbf{Overhead} 
\\
%\cline{2-4} 
\hline
\hline
\begin{tabular}[c]{@{}c@{}}
Dense RF with \\
Dense SA
\end{tabular}

& X
& X
& None
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Sparse RF with \\
Dense SA
\end{tabular}
& O
& X
& Indexing logic
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Dense RF with\\
Sparse SA
\end{tabular}
& X
& O
&
Interconnection
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Sparse RF with\\
Sparse SA
\end{tabular}
& O
& O
&
\begin{tabular}[c]{@{}c@{}}
Indexing logic, \\
interconnection
\end{tabular}
\\
\hline

\end{tabular}
\label{tab1}
\label{table:sa-tradeoff}
\end{table}
